Decentralizing Centralized Matching Markets: Implications from Early Offers in University Admissions

The matching literature often recommends market centralization under the assumption that agents know their own preferences and that their preferences are fixed. We find counterevidence to this assumption in a quasi-experiment. In Germany's university admissions, a clearinghouse implements the early stages of the Gale-Shapley algorithm in real time. We show that early offers made in this decentralized phase, although not more desirable, are accepted more often than later ones. These results, together with survey evidence and a theoretical model, are consistent with students' costly learning about universities. We propose a hybrid mechanism to combine the advantages of decentralization and centralization. Published at The Journal of Political Economy under a new title, ``Preference Discovery in University Admissions: The Case for Dynamic Multioffer Mechanisms,'' available at https://doi.org/10.1086/718983 (Open Access).

==> Style/Macros.tex <==
\makeatletter
\g@addto@macro{\clearpage}{\nointerlineskip}
\makeatother

\makeatletter
\AtBeginEnvironment{appendices}{%
  \clearpage
  \addcontentsline{toc}{chapter}{Appendices}
  \write\@auxout{%
    \string\let\string\latex@tf@toc\string\tf@toc% Store the original `\tf@toc` file handle
    \string\let\string\tf@toc\string\tf@apc%
  }% Naughty trick
\titleformat{\section}{\bfseries}{\Large\thesection}{0.8em}{\Large}
\titlespacing*{\section}{0pt}{0pt}{2.3ex plus .2ex}
}
\AtEndEnvironment{appendices}{%
  \write\@auxout{%
    \string\let\string\tf@toc\string\latex@tf@toc%
  }% Naughty trick, restoring the old `\tf@toc` number, to be able to write stuff to the real `.toc` again.
}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             CUSTOMIZATION                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% To define argmin, argmax
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% early offer
\DeclareMathOperator{\EarlyOffer}{\mathit{EarlyOffer}}
\DeclareMathOperator{\FirstEarlyOffer}{\mathit{FirstEarlyOffer}}
\DeclareMathOperator{\Accept}{\mathit{Accept}}
\DeclareMathOperator{\EO}{\it EO}
\DeclareMathOperator{\FEO}{\it FEO}
\DeclareMathOperator{\EU}{EU}

% math notations
\def\P{\mathbb{P}}
\def\E{\mathbb{E}}

%% reminders

% put \mute{ok} to mute comments
\def\mute{ok}
\def\ok{ok}

% Muted comments except changes
\ifx\mute\ok
\newcommand{\reminder}[1]{} % show all the reminders

% Visible comments
\else
\newcommand{\reminder}[1]{\textcolor{blue}{** #1 **}} % show all the reminders
\fi

\newcommand{\red}[1]{\textcolor{red}{#1}} % highlight in red
\newcommand{\orange}[1]{\textcolor{orange}{#1}} % highlight in red
\newcommand{\blue}[1]{\textcolor{blue}{#1}} % highlight in red

\definecolor{chicago-maroon}{RGB}{128,0,0}
\newcommand{\yh}{\textcolor{chicago-maroon}}

% To create environments for definitions, theorems, etc.
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{prop}{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}

\linespread{1.5}

% Customize margins
\geometry{left=1in, right=1in, top=1in, bottom=1in}

% To avoid the warning message when including pdf files %
\pdfoptionpdfinclusionerrorlevel=0
\pdfoptionpdfminorversion=6

% Caption style
\captionsetup{font=normalsize,labelfont=bf}
\captionsetup[table]{labelsep=endash}
\captionsetup[figure]{position=bottom,labelsep=endash}

% Thickness of table rules %
\setlength{\heavyrulewidth}{0.11em}

% Customize date format
%\newdateformat{dashdate}{\monthname[\THEMONTH] \THEYEAR}

% USER-DEFINED MACROS

% \graphique: to include figures in pdf
\newcommand{\graphique}[2][1]{\begin{minipage}{\linewidth}\begin{center}\includegraphics[width=#1\linewidth,clip]{Figures/#2}\end{center}\end{minipage}}

% TABNOTES: environment for table notes
\newenvironment{tabnotes}[2][1]{\begin{minipage}[t]{#1\textwidth}\vspace{0.1cm}\scriptsize{\emph{Notes:} #2}}{\end{minipage}}

% Customize appendix
\newcommand{\listappendixname}{List of Appendices}
\newlistof{appendix}{apc}{\listappendixname}
\setcounter{tocdepth}{2}



% Bookmark (signets): to have numbered and unnumbered bookmarks
%https://tex.stackexchange.com/questions/232399/section-numbers-in-pdf-bookmarks
\makeatletter
\newcommand{\numbersections}{\renewcommand{\Hy@numberline}[1]{##1. }}
\newcommand{\nonumbersections}{\renewcommand{\Hy@numberline}[1]{}}
\makeatother

\newcolumntype{C}{>{\Centering\arraybackslash}X}
\newcommand\mc[1]{\multicolumn{1}{c}{#1}} % handy shortcut macro
\newcommand\mC[1]{\multicolumn{1}{C}{#1}} % handy shortcut macro

\newcolumntype{R}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{B}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{T}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% symbols

\def\J{\mathcal{J}}
\def\U{\mathcal{U}}
\def\oU{\overline{\mathcal{U}}}
\def\NR{\mathcal{NR}}
\def\T{\mathcal{T}}
\def\ut{\underline{t}}

% Missing references
\makeatletter
\patchcmd{\@setref}{\bfseries ??}{\colorbox{red}{?reference?}}{}{}%
\patchcmd{\@citex}{\bfseries ?}{\colorbox{red}{?citation?}}{}{}%
\makeatother

% Date format
\newdateformat{dashdate}{\monthname[\THEMONTH] \THEYEAR}

